RELICS-DP7: Spectroscopic Confirmation of a Dichromatic Primeval Galaxy at z ~ 7

We report the discovery of a spectroscopically-confirmed strong Lyman-$\alpha$ emitter at $z=7.0281\pm0.0003$, observed as part of the Reionization Cluster Lensing Survey (RELICS). This galaxy, dubbed "Dichromatic Primeval Galaxy" at $z\sim7$ (DP7), shows two distinct components. While fairly unremarkable in terms of its ultraviolet (UV) luminosity ($\sim0.3L^{\ast}_{UV}$, where $L^{\ast}_{UV}$ is the characteristic luminosity), DP7 has one of the highest observed Lyman-$\alpha$ equivalent widths (EWs) among Lyman-$\alpha$ emitters at $z>6$ ($>200$ Angstrom in the rest frame). The strong Lyman-$\alpha$ emission generally suggests a young metal-poor, low-dust galaxy; however, we find that the UV slope $\beta$ of the galaxy as a whole is redder than typical star-forming galaxies at these redshifts, $-1.13\pm 0.84$, likely indicating, on average, a considerable amount of dust obscuration, or an older stellar population. When we measure $\beta$ for the two components separately, however, we find evidence of differing UV colors, suggesting two separate stellar populations. Also, we find that Lyman-$\alpha$ is spatially extended and likely larger than the galaxy size, hinting to the possible existence of a Lyman-$\alpha$ halo. Rejuvenation or merging events could explain these results. Either scenario requires an extreme stellar population, possibly including a component of Population III stars, or an obscured Active Galactic Nucleus. DP7, with its low UV luminosity and high Lyman-$\alpha$ EW, represents the typical galaxies that are thought to be the major contribution to the reionization of the Universe, and for this reason DP7 is an excellent target for follow-up with the James Webb Space Telescope.

==> DP7_ ApJL_final/DP7_mags_no_mucorr.tex <==
\begin{deluxetable}{cccc}
\tabletypesize{\footnotesize}
\tablecaption{DP7 HST and Spitzer Photometry} 
\tablehead{
\colhead{\hspace{0.15cm}Filter}\hspace{0.15cm}  & \colhead{\hspace{0.15cm}Whole Galaxy}\hspace{0.15cm}  & \colhead{\hspace{0.15cm}North Component}\hspace{0.15cm} & \colhead{\hspace{0.15cm}South Component}\hspace{0.15cm}
} 
\startdata
F435W & $>28.8$         &  $>29.0$          &  $>31.5$\\
F606W & $>29.7$         &  $>30.2$          &  $>30.0$\\
F775W & $>28.7$         &  $>29.1$          &  $>29.0$\\
F105W & $27.16\pm0.15$  &  $28.02\pm0.22$   & $27.81\pm0.21$\\
F125W & $28.26\pm0.78$  &  $28.08\pm0.44$   &  $>28.9$\\
F140W & $27.21\pm0.28$  &  $27.96\pm0.36$   & $27.97\pm0.42$\\
F160W & $27.18\pm0.20$   &  $28.45\pm0.42$   &  $27.57\pm0.22$\\
$$\rm{[3.6]}$$ &  $25.4\pm0.3$  &  $--$   & $--$ \\
$$\rm{[4.5]}$$ & $25.3\pm0.4$   &  $--$   & $--$ \\
\enddata

\tablenotetext{}{We report AB magnitudes measured in HST and Spitzer images of DP7 as a whole galaxy and as two separated components, except for the Spitzer images from which we measure only magnitudes for the whole galaxy (see Section~\ref{subsec:imaging}). The magnitudes are measured in isophotal apertures shown in the inset of Figure~\ref{fig:hstimage}. }

\end{deluxetable}


==> DP7_ ApJL_final/properties.tex <==
\begin{deluxetable}{cc}
\tabletypesize{\footnotesize}
\tablecaption{\label{tbl-1} Summary of DP7 Properties} 
\tablehead{
\colhead{\hspace{1.35cm}Property}\hspace{1.35cm}  & \colhead{\hspace{1.35cm}Value}\hspace{1.35cm}
} 
\startdata
RA (Deg.) & 152.6593385 \\
Dec (Deg.) & -12.6556351 \\
$z$& $7.0281\pm0.0003$ \\
$\mu$ & $1.15\pm0.2$\\
$\rm{M}_{\rm{stellar}}$  ($10^9M_{\odot}$) & $4.9^{+3.8}_{-3.2}$\\
SFR ($M_{\odot} \rm{yr}^{-1}$) & $11.2^{+10.3}_{-7.2}$ \\ 
sSFR ($\rm{Gyr}^{-1}$) & $2.1^{+5.2}_{-2.4}$\\
E(B-V) (mag) & $0.15\pm0.10$\\
$\rm{M}_{\rm{UV}}$ (mag) &  $-19.5\pm 0.2$\\
$\mathrm{L(Ly\alpha) (erg\,s^{-1})}$ & $1.0\pm 0.1 \times 10^{43}$\\
Ly$\alpha$ EW$_{\rm{F105W}}$ (\AA) & $237.12\pm 57.78$\\
Ly$\alpha$ EW$_{\rm{F140W}}$ (\AA) & $341.55\pm 93.78$\\
Ly$\alpha$ FWHM (\kms) & $285.3^{+23.9}_{-76.4}$ \\
Ly$\alpha$ size (kpc) & $2.09\pm 0.88$\\
F160W size (kpc) & $0.56\pm 0.20$\\
\enddata

\tablenotetext{}{$\mu$ is the magnification factor: median magnification and 68\% confidence limits from the MCMC lens model uncertainties. $\mu=\mu_{\rm{med}}$ is assumed in SFR,  $\rm{M}_{\rm{stellar}}$, and $\rm{M}_{\rm{UV}}$ calculations. Uncertainties include statistical 68\% CLs from photometry and redshift. To use a different magnification value, multiply the quantity by $1/f_{\mu}$, where $f_{\mu}\equiv\mu/\mu_{\rm{med}}$. $\rm{M}_{\rm{stellar}}$ is the intrinsic stellar. sSFR is the specific SFR, sSFR $\equiv M_{stellar}$/SFR. E(B-V) is dust color excess of stellar emission. SMC dust law assumed. $\rm{M}_{\rm{UV}}$ is rest-frame UV magnitude assuming $\mu{\rm_{med}}$, derived from the observed F160W magnitude including a small template-based $k$-correction. To use a different magnification value, use $\rm{M}_{\rm{UV}}-2.5\rm{log}(f_{\mu}$). Ly$\alpha$ FWHM is measured non-parametrically by estimating the wavelength at which the line drops to 50\% of the peak on the blue and red side. The FWHM error is estimated by a Monte-Carlo technique.}

\end{deluxetable}
